Theory of Regulatory Compliance for Requirements Engineering

Regulatory compliance is increasingly being addressed in the practice of requirements engineering as a main stream concern. This paper points out a gap in the theoretical foundations of regulatory compliance, and presents a theory that states (i) what it means for requirements to be compliant, (ii) the compliance problem, i.e., the problem that the engineer should resolve in order to verify whether requirements are compliant, and (iii) testable hypotheses (predictions) about how compliance of requirements is verified. The theory is instantiated by presenting a requirements engineering framework that implements its principles, and is exemplified on a real-world case study.

==> introduction.tex <==
\section{Introduction}\label{s:introduction}

A legal norm (aka law, regulation) is a body of knowledge that acts both as a source of requirements and as a filter for requirements. Just as any requirement can be considered desirable or undesirable, it is also either compliant or not with relevant law, whereby compliance of a requirement refers informally to its alignment to law. Determining whether some set of requirements is compliant with relevant laws is therefore becoming a central issue in Requirements Engineering (RE). This was to be expected, for non-compliant requirements result in -- quite literally -- an illegal information system, thereby risking sanctions for their owners and users, among others. An RE project certainly cannot purport to be successfully executed if it fails to establish regulatory compliance.

Verifying and ensuring regulatory compliance is a difficult problem fought continually in and out of courtrooms  with large budgets, over long periods of time. It should not be expected of the legislators who author laws to reduce either these budgets or time spans. Rather, the challenge is on the designers of information systems, and thus on requirements engineers who must at the very outset of the information systems engineering effort verify through a systematic process that requirements indeed comply with relevant laws. To do so, they need methods, and methods in turn require that we are clear on what regulatory compliance means in the first place. 

This paper offers a theory of regulatory compliance and discusses its application via a real-world compliance problem. The theory starts from simple observations, prima facie evidence on how compliance is being engineered into systems, providing as a result the so-called compliance relation $\nmc_{C}$ between a requirements specification and set of norms. The compliance relation comes together with: (i) formal pragmatic conditions that requirements should satisfy in order to be considered compliant; (ii) a formal definition of the compliance problem, i.e., the problem that the engineer should resolve in order to verify that requirements are compliant; (iii) testable hypotheses about how regulatory compliance of requirements is verified.

The proposed framework is founded on argument-theoretic, as opposed to truth-theoretic, semantics. This means that compliance is not reduced to establishing that if requirements along with assumptions are ``true'' so is the norm with respect to which we are establishing compliance. Rather, compliance means that an argument that a given set of requirements complies with a given norm, is ``acceptable''
%provided certain assumptions are ``acceptable'' 
to stakeholders. The argumentation concepts used are adopted from~\cite{jur-myl-faul-RE09}, though in somewhat simplified form.

The rest of the paper is structured as follows. We start with an informal discussion of what it means for requirements to be compliant with some relevant law (\S2). The three parts of the compliance theory for requirements are then presented and discussed in detail (\S3). A requirements engineering framework is presented, which provides an implementation of the theory (\S4--5). The theory is applied via an example of a real-world compliance problem (\S6). The paper closes with the discussion of related work (\S7), a summary of conclusions, and pointers for future research (\S8).




==> process.tex <==
\section{The compliance process}\label{s:case-study}

The \nomos language allows for building models of requirements that comply with law according to the theory described in section~\ref{s:theory}. This is done through a process, which takes into consideration: (i) the production of a compliance solution; (ii) the argumentation supporting (or attacking) such solution; and (iii) the algorithm for making conclusions from the argumentation. The three corresponding phases form an iterative process, in which argumentation moves from the modeled solution and may require to change it, until the algorithm allows for deducing compliance acceptance.

\paragraph{\B{Phase 1. Compliance modeling}} 
%Given a set of requirements $R$ and a set of NPa $L$, a solution is found for every NP.
%
%\B{Phase 2}. Once a compliance solution is found, it is presented to the stakeholders for evaluation.
%
%\B{Phase 3}.
%
It basically consists in the application of the \nomos modeling process.
%, which starts from a model $L$ of law and a model $R$ of requirements, and ends with a new requirements set, $R^\prime$, which is compliant with $L$ under a set of compliance assumptions $C$.
%
%In \nomos, compliance is established through a modeling process, which starts from a model $L$ of law, represented as a set of normative propositions $\lbrace \np_1$, ..., $\np_{nn} \rbrace$, and a model $R$ of requirements, represented as a set of goals $\lbrace g_1$, ..., $g_{gn} \rbrace$, and ends with a new requirements set, $R^\prime$, which is compliant with $L$ under a set of compliance assumptions $C$.
The methodological aspects of the process are described in detail in~\cite{sie-myl-per-susi-ER09}:
the process is basically comprised by various steps, each of them starting by arguing a compliance issue, and ending with agreement on the solution for that issue.
For the purpose of this paper, we will focus on those parts of the process, which deal with the actual establishment of the compliance condition, without considering law modeling aspects mentioned in~\cite{sie-myl-per-susi-ER09}.


\newcounter{steps}

\noindent \refstepcounter{steps}\label{step:binding}\arabic{steps}. \I{Identify applicable laws}.
%
Each NP addresses a subject. If a certain actor of the domain is subject to the NP, the NP is applicable to it and it has to comply w.r.t. the NP. 
%The binding between domain stakeholders and legal subjects has to be preliminary identified in~\cite{sie-myl-per-susi-ER09} as a necessary step is to bind domain stakeholders with legal subjects. 
For example, if the law addresses a ``Covered Entity'' (CE), and a stakeholder of the domain is a Hospital, we have to decide if the Hospital is (or not) a CE. In the first case, the NPs of the law apply to the Hospital, and it has to be compliant. 
%
If an actor is agreed to be a certain legal subject, this information is added to the argumentation tree.


\noindent \refstepcounter{steps}\label{step:apply}\arabic{steps}. \I{Identify affected goals}.
Each NP applicable to a given actor can affect the actor's strategy. A NP is not affecting a strategic goal if the achievement of the goal, no matter \textit{how} it is achieved, does not allow for a violation of the NP. If, according to how a goal is achieved, the NP can be violated or respected, the goal needs to be elaborated for compliance. 


\noindent \refstepcounter{steps}\label{step:realize}\arabic{steps}. \I{Choose realizing goals}.
% <IVAN>
A compliance goal appears in an actor's rationale because the actor must be compliant with some NP.
A top-level compliance goal realizes a NP --- i.e., there is a realization relation from that goal to the NP, meaning that satisfying that goal satisfies the NP, and indicates compliance with that NP.
The realization relation results in practice in that the NP that the goal realizes is a constraint on the definition of the solution for that goal: any solution for the goal must be such that the realization relation is not violated, i.e., that it is not dropped by a solution because that solution satisfies the goal in a way that violates the NP. 
%A compliance goal is a goal, whose reason-to-be within an actor's rationale is the need for the actor to be compliant with a normative proposition.
%With respect to the normative proposition, a top-level compliance goal is its realizing goal --- i.e., a goal that is put in realization relation with the normative proposition; this means that the goal is hypothesized to allow compliance with the normative proposition.
%The realization relation becomes then a desired constraint over the goal's achievement: the subsequent modeling of a solution for the goal must be such that the realization relation holds --- i.e., iff in the belief of the actor the achievement of the goal implies its compliance. So the ``iff'' condition bounds the semantics of the goal with its expected operationalization into tasks. The realizing goal is an abstraction for the solution to the normative proposition, and we add it to the set of requirements $R$, while the realization relation is added to the compliance assumptions $C$.
% </IVAN>


\noindent \refstepcounter{steps}\label{step:refine}\arabic{steps}. \I{Refine compliance goals}.
% <IVAN>
A compliance goal must be refined in such a way that every alternative refinement thereof must not violate the NP that this compliance goal realizes. Subgoals in the refinements must be chosen in such a way that their joint satisfaction does not violate the NP.
%In order for a realization relation to hold, the realizing goal has (generally, but not necessarily) to be further constrained in its semantics. A goal is constrained in semantics by means of modeling choices, such as the refinement of the goal into sub-goals, or the delegation of its achievement to other actors. By performing such actions, further semantic constraints are added to the possible solution for the goal.
% </IVAN>


\noindent \refstepcounter{steps}\label{step:operationalize}\arabic{steps}. \I{Operationalize compliance goals}.
If $g$ is a compliance goal for a given NP, a solution for it has to be 
% <IVAN>
sought by refining/decomposing $g_k$ onto subgoals, then finding tasks the execution of which satisfies the subgoals.
If $g$ is AND-refined/decomposed onto subgoals $g_{1}$ and $g_{2}$, then $g$ is compliant if and only if the conjunction of the two subgoals %, i.e., $g_{1} \wedge g_{2}$ 
is compliant:
%Obviously, 
neither the satisfaction of $g_{1}$ alone, nor of $g_{2}$ alone is good enough to ensure that $g$ is satisfied. 
In general terms, the solution $sol(g)$ for the compliance goal $g$ is the conjunction of its leaf tasks.
%In general terms, if a goal $g$ is AND-refined onto subgoals $g_{1}, \ldots, g_{n}$, then all subgoals must be satisfied together, so that if every subgoal $g_{i}$ is AND-operationalized by the tasks $t_{i,1}, \ldots, t_{i,m_{i}}$, then the conjunction $t_{i,1} \wedge \ldots \wedge t_{i,m_{i}}$ of these tasks must be executed (i.e., all of these tasks must be executed) in order to satisfy $g_{i}$. Stated otherwise, in order to satisfy $g$, we must execute all tasks $t_{1,1}, \ldots, t_{n,m_{n}}$.
% </IVAN>

%searched by decomposing $g$ until finding a task set. If $g$ is AND-decomposed into two sub-goals $sg_1, sg_2$, for the purpose of this work we assume that the compliance of $g$ is equivalent to the compliance of $sg_1 \AND sg_2$. Neither the achievement of $sg_1$, nor the achievement of $sg_2$ is enough to argue about compliance. Only the achievement of both sub-goals could allow to fulfil the normative proposition. Otherwise, Step \arabic{steps} has to be iterated. To generalize, in a decomposition tree with $g$ as top goal and $t_1, ..., t_n$ as leaf tasks, $sol_S(g) = \bigwedge_{k=1}^n{t_k}$; $sol_S(g)$ is one of the possible solutions for $g$ and belongs to $Spec(R)$.


\noindent
\textit{Outcomes}.
% <IVAN>
%We have previously defined (in Definition~\ref{d:complianceproblem}) the compliance problem in argumentation terms as: 
%Definition III.17 stated the compliance problem in argumentation terms as:
%% </IVAN>
%$\textit{Spec}(R), C \nmc_{C} L$.
%We have introduced the set of requirements $R = \lbrace g_1, ..., g_{gn} \rbrace$, and the set of NPs $L = \lbrace \np_1, ..., \np_{ln} \rbrace$. We have refined the goals into tasks so that $Spec(R) = \lbrace t_1, ... t_{tn} \rbrace$ is the solution for $R$. The compliance assumptions $C$ are defined as a set of ``realization'' relations that bound $R$ and $L$.
%The compliance connective $\nmc_{C}$ states that the compliance assumptions ensure compliance of requirements with respect to the given laws, and this assertion is justified with the argumentation that led to the construction of $C$.
%
Definition III.17 stated the compliance problem in argumentation terms as: $\textit{Spec}(R), C \nmc_{C} L$.
%The described process ends up with a model of $L$ and a model of $Spec(R)$
%
After the application of the described process, we have that:
$L$ is the input model of the law we want to address;
$R$ is the initial requirements set, refined in the steps 3 and 4;
$Spec(R)$ amounts in the solution for $R$ - i.e., the sets of tasks that operationalize the compliance goals;
$C$ contains the set of realization relations. %The next phase concerns the establishment of the $\nmc_{C}$ relation.
%
The compliance condition expressed by the $\nmc_{C}$ relation can't however be formally proved. Rather, it has to be argued by providing evidence that the compliance modeling choices are reasonably acceptable.

\paragraph{\B{Phase 2. Argumentation}}
%Recalling the theory, $\phi_R$ is the set of well-formed sentences on $R$ and $\psi_L$ is the set of well-formed sentences on $L$, and $\phi_C$ is a set of well-formed sentences on $C$. 
The compliance of the framework is deduced form the dialectical tree $T(a(\phi))$. The tree is primarily formed by the arguments collected during phase 1 of the process. For example, if a goal delegation resulted from a consideration on the abilities of the delegatee in fulfilling the goal, such considerations are added to the argumentation as a support that that modeling choice.
Phase 2 consists in debating about the modeling choices. Three types of argument can be given:\\
(i) Arguments in favor of the modeling choices; i.e., arguments that confirm the conclusions of the argumentation tree built during the development of the solution (phase 1).\\
(ii) Arguments in favor of for changing or replacing some parts of the solution; in this case, such arguments are added to the argumentation tree, and a modeling activity is undertaken again to change $R$ into an $R^\prime$.\\
(iii) Arguments that reject partly or completely the conclusions of the argumentation tree; in this case, a new solution for $L$ has to be searched.
%
%If other arguments are raised, for example by the stakeholders, which conflict with the modeling choices, such arguments are added as well to the argumentation tree, until no new arguments can be found, in favor or against the modeled compliance solution.
%So ultimately we can state that, because of the argumentation $\Gamma$, the compliance assumptions $C$ ensure the requirements $R$ to be compliant with the laws $L$. In the next section, we will exemplify how the argumentation is framed.


\paragraph{\B{Phase 3. Verification}}
The dialectical tree can be traversed for making conclusions form it by means of a justification process as described in Definition III.16.
The process starts from the leaves and makes conclusions on the acceptability of the roots, which are basically the compliance hypotheses (as of step 3 of phase 1).
If the justification process allows for deducing acceptance of the compliance hypotheses, then compliance is demonstrated on an argumentation basis. If compliance can be demonstrated for every NP, we say that the requirements  $R$ are compliant with the law $L$. If new arguments come in, the validity of a conclusion is not ensured anymore, and the process has to be iterated.

%The process starts from the leaves (which are true because they are not attacked by anything) and going up to the roots. If the root compliance arguments are not labeled false, we say that compliance is argued. Otherwise, the process has to be iterated, by adding, removing or replacing requirements, or by revising the argumentation.
%When there is nothing else to be added to the the dialectical tree, it ends up in containing all the information in favor or against the validity of the compliance condition between the requirements and the law. 







==> relatedworks.tex <==
\section{Related Works}\label{s:related-work}

Allen~\cite{allen-57} firstly pointed out the possibility to formalize law as a logical theory, in order to be able to make conclusions about the consequences of the law.
%
%Law firstly came into the scene of computer science with the efforts made by logicians to represent legal prescriptions in a formal shape. The idea, pointed out by Allen~\cite{allen-57} was that it is possible to formalise law as a logical theory, in order to be able to make conclusions about the consequences of the law.
%
Worth mentioning in particular Stamper's LEGOL~\cite{stamper-80}, a LEGally Oriented Language aimed at expressing a legislation by means of formal rules, suitable to be processed by computers. The idea behind LEGOL was that legislations shape the behaviour of information systems: regardless on \textit{how} information systems are implemented, they perform within the boundaries created by laws.
%
%McCarty's TAXMAN system~\cite{mccarty-80} is an (experimental) application of artificial intelligence techniques to the study of legal reasoning and legal argumentation, using corporate tax law as problem domain.
%It allows to build models of facts comprising tax-related cases, such as corporations issue securities, transfer property, distribute dividends, and so on. Law (specifically: the United States Internal Revenue Code) is represented as rules, which classify transactions as taxable or nontaxable, ordinary income or capital gains, dividend distributions or stock redemptions, etc.
%Testing on several stock dividend and corporate reorganization cases decided by the Supreme Court in the 1920's and 1930's.
%
%Following this experimental work, McCarty developed a Language for Legal Discourse (LLD)~\cite{mccarty-ICAIL89}, based on deontic logic, to specify actions as well as deontic operators. In LLD, one can specify the rule that any corporation that owns cash has an obligation to distribute cash to all its stockholders in a Lisp-like syntax.
%
%A well known example of this approach is the work by Kowalski et al., who try to represent the British Nationality Act as a logic program~\cite{ser-sad-kow-kru-ham-cory-ACM86}. That approach has been reported to be successful in the given context, suggesting the feasibility for its application to a larger class of cases.

In recent years, law compliance has increasingly been addressed in relation with requirements engineering.
Anton and Breaux have developed a systematic process, called semantic parameterisation, which consists of identifying in legal text restricted natural language statements (RNLSs) and then expressing them as semantic models of rights and obligations~\cite{bre-vail-ant-re06} (along with auxiliary concepts such as actors and constraints). 

Darimont and Lemoine have used KAOS as a modelling language for representing objectives extracted from regulation texts~\cite{dar-lem-ReMo2V06}. Such an approach is based on the analogy between regulation documents and requirements documents. Ghanavati et al.~\cite{gha-am-pey-RE09} use GRL to model goals and actions prescribed by laws. This work is founded on the premise that the same modelling framework can be used for both regulations and requirements.  Likewise, Rifaut and Dubois use \textit{i*} to produce a goal model of the Basel II regulation~\cite{rif-dub-RE08}.




